All-Norm Load Balancing in Graph Streams via the Multiplicative Weights Update Method

In the weighted load balancing problem, the input is an $n$-vertex bipartite graph between a set of clients and a set of servers, and each client comes with some nonnegative real weight. The output is an assignment that maps each client to one of its adjacent servers, and the load of a server is then the sum of the weights of the clients assigned to it. The goal is to find an assignment that is well-balanced, typically captured by (approximately) minimizing either the $\ell_\infty$- or $\ell_2$-norm of the server loads. Generalizing both of these objectives, the all-norm load balancing problem asks for an assignment that approximately minimizes all $\ell_p$-norm objectives for $p \ge 1$, including $p = \infty$, simultaneously. Our main result is a deterministic $O(\log{n})$-pass $O(1)$-approximation semi-streaming algorithm for the all-norm load balancing problem. Prior to our work, only an $O(\log{n})$-pass $O(\log{n})$-approximation algorithm for the $\ell_\infty$-norm objective was known in the semi-streaming setting. Our algorithm uses a novel application of the multiplicative weights update method to a mixed covering/packing convex program for the all-norm load balancing problem involving an infinite number of constraints.

==> distributed.tex <==
\section{Distributed Load Balancing}

\begin{definition}
  The \emph{client-replicated graph} is the graph formed by making $w(c)$
  copies of each client $c$.
\end{definition}

\begin{definition}
  Let $\tilde{G}$ be the client-replicated graph of $G$.
  Let $A^*$ be the all-norm optimal assignment of $\tilde{G}$ with the
  lexicographically smallest load vector.
  Let $C_i^*$ be the set of clients in $\tilde{G}$ that are adjacent to a
  server of load at most $i$ in $A^*$.
  The \emph{level} of a client $c$ is the minimum $i$ such that $c \in C_i^*$.
\end{definition}

\begin{definition}
  A \emph{level-$\ell$ assignment} is an $x : E \to \nonneg$ such that
  $x(\delta(c)) = w(c)$ for all $c \in C$.
  The maximum load of a level-$\ell$-assignment is $\max_{c \in C} x(\delta(c))$.
\end{definition}

\begin{lemma}
  If there is an algorithm to compute a level-$\ell$-assignment of load $\alpha
  \ell$, then there is an algorithm to compute a $4\alpha$-approximate solution
  to the all-norm load balancing problem.
\end{lemma}
\begin{proof}
  Compute a level-$2^i$ assignment $x_i$ for $i \in \{0, \dots, \log_2 n\}$ such
  that $x_i$ has maximum load $\alpha 2^i$.
  Each client then greedily assigns itself, starting from $x_0$, until all of
  its units have been assigned.

  Fix a server $s$ and let $\ell$ be the smallest nonnegative integer such that
  $x^*(\delta(s)) \le 2^\ell$.
  By definition, $N(s) \subseteq C_\ell$.
  Since $x_\ell$ is a level-$2^\ell$ assignment, it saturates every client in
  $C_\ell$, and in particular, every client in $N(s)$.
  Hence no edges from $x_i$ for $i > \ell$ are used in the assignment of $s$.
  Hence \[
    x(\delta(s)) \le \sum_{i=0}^\ell x_i(\delta(s)) \le \sum_{i=0}^\ell \alpha 2^i \le 4 \alpha \cdot 2^{\ell-1} \le 4\alpha x^*(\delta(s)).
  \]
  It follows that $\lVert L_x \rVert \le 4\alpha \cdot \lVert L_{x^*} \rVert$.
\end{proof}

\begin{figure}[ht]
  \begin{algorithm}[H]
    Compute a level-$2^i$-assignment $x_i$ for $i \in \{0, \dots, \log_2{n}\}$.\;
    Merge $x_i$ greedily to form a $(w, w(C))$-matching.
  \end{algorithm}
\end{figure}

\begin{figure}[ht]
  \begin{algorithm}[H]
  Set $x(e) \gets 0$ for all $e \in E$.\;
  Set $b(c) \gets w(c)$ for all $c \in C$.\;
  Set $b(s) \gets \ell$ for all $s \in S$.\;

  \For{$j \gets 0$ \KwTo $\jmax$}{
    Compute a maximal $b$-matching $y$ of $\Gj$.\;
    Set $x(e) \gets x(e) + y(e)$ for all $e \in \Ej$.\;
    Set $b(v) \gets b(v) - y(\delta(v))$ for all $v \in V$.\;
  }
  Set $z(cs) \gets 2x(cs) / w(c)$.\;
  Return $z$.\;
\end{algorithm}
\end{figure}

\begin{lemma}
  Let $x$ be the value computed at the end of the algorithm.
  Then $x$ restricted to $\Ej$ is a maximal $(w, \ell)$-matching of
  the graph $(C, S, \Ej)$ for all $j \in \{0, \dots, \jmax\}$.
\end{lemma}
\begin{proof}
  In general, if $x$ is a maximal $b_1$-matching and $y$ is a maximal $b_2$
  matching, then $x + y$ is a maximal $(b_1 + b_2)$-matching.

  The algorithm maintains the following precondition on the loop:
  at the beginning of iteration $j$ we have $b(c) = w(c) - x(\delta(c))$ for $c
  \in C$ and $b(s) = \ell - x(\delta(s))$ for $s \in S$.
  It follows that $x$ is a maximal $(w, \ell)$-matching of $\Gj$ at the end
  of iteration $j$.
\end{proof}

\begin{lemma}
  Let $z$ be the value returned by the algorithm.
  Then \[
    \sum_{c \in C^*_\ell} \lambda(c) z(\delta(c)) \ge \sum_{c \in C^*_\ell} \lambda(c).
  \]
\end{lemma}
\begin{proof}
  We have \begin{align*}
    \sum_{c \in C^*_\ell} \lambda(c) z(\delta(c))
    &= 2 \sum_{c \in C^*_\ell} \rho(c) x(\delta(c))\\
    &= 2 \sum_{j=0}^\jmax \sum_{c \in C^*_\ell \cap \Cj} \rho(c) x(\delta(c))\\
    &\ge 2 \sum_{j=0}^\jmax (r_j - r_{j-1}) x(\Ej_\ell)\\
    &\ge \sum_{j=0}^\jmax \sum_{c \in C^*_\ell \cap \Cj} (r_j - r_{j-1})x^*(\Ej_\ell)
    &= \sum_{j=0}^\jmax \sum_{c \in C^*_\ell \cap \Cj} (r_j - r_{j-1})x^*(\Ej_\ell)
  \end{align*}
\end{proof}

